Markov-Equivalent Conditional Independence Graphs on Path Spaces

Causal discovery for continuous-time stochastic processes with latent confounding typically faces a trade-off between (i) approaches that are highly informative about the causal structure but are difficult to test statistically, and (ii) approaches that admit practical tests from data but yield more coarse-grained conclusions, potentially not leveraging the direction of time. We introduce W-separation, an asymmetric graphical criterion for directed mixed graphs defined as a quaternary relation that allows distinct conditioning on past and future components. This added flexibility yields a highly informative graphical independence model while preserving testability. W-separation satisfies a global Markov property for a broad class of stochastic differential equations with latent confounding, linking it to conditional independence relations among coordinate processes that are testable from data. A central result of this work is the full characterization of W-Markov equivalence classes: we show that every equivalence class admits a unique greatest element that serves as a canonical representative and a principled target for learning algorithms. In addition, we provide necessary and sufficient conditions under which directed or bidirected edges can be added without altering the induced independence model.

==> preamble.tex <==
\usepackage{tikz-cd}
\usetikzlibrary{%
    arrows,calc,shapes,positioning}

\RequirePackage{enumitem}
\RequirePackage{mathtools}

\RequirePackage{%
    amssymb,mathrsfs,bm}

\let\theorem\relax
\let\lemma\relax
\let\proposition\relax
\let\corollary\relax

\let\definition\relax
\makeatletter
\let\remark\@undefined
\let\endremark\@undefined
\makeatother

\usepackage{amsthm}
\usepackage{thmtools}
\declaretheorem[name=Theorem, refname={Theorem,Theorems}, Refname={Theorem,Theorems}, numberwithin=section]{theorem}
\declaretheorem[name=Lemma, refname={Lemma,Lemmas}, Refname={Lemma,Lemmas}, sibling=theorem]{lemma}
\declaretheorem[name=Proposition, refname={Proposition,Propositions}, Refname={Proposition,Propositions}, sibling=theorem]{proposition}
\declaretheorem[name=Corollary, refname={Corollary,Corollaries}, Refname={Corollary,Corollaries}, sibling=theorem]{corollary}

\declaretheorem[name=Definition, refname={Definition,Definitions}, Refname={Definition,Definitions}, sibling=theorem]{definition}
\declaretheorem[name=Assumption, refname={Assumption,Assumptions}, Refname={Assumption,Assumptions}, sibling=theorem]{assumption}
\declaretheorem[name=Remark, numbered=no]{remark}

\RequirePackage[capitalize,nameinlink,noabbrev]{cleveref}

\crefname{enumi}{}{}

